TCDM Burst Access: Breaking the Bandwidth Barrier in Shared-L1 RVV Clusters Beyond 1000 FPUs

As computing demand and memory footprint of deep learning applications accelerate, clusters of cores sharing local (L1) multi-banked memory are widely used as key building blocks in large-scale architectures. When the cluster's core count increases, a flat all-to-all interconnect between cores and L1 memory banks becomes a physical implementation bottleneck, and hierarchical network topologies are required. However, hierarchical, multi-level intra-cluster networks are subject to internal contention which may lead to significant performance degradation, especially for SIMD or vector cores, as their memory access is bursty. We present the TCDM Burst Access architecture, a software-transparent burst transaction support to improve bandwidth utilization in clusters with many vector cores tightly coupled to a multi-banked L1 data memory. In our solution, a Burst Manager dispatches burst requests to L1 memory banks, multiple 32b words from burst responses are retired in parallel on channels with parametric data-width. We validate our design on a RISC-V Vector (RVV) many-core cluster, evaluating the benefits on different core counts. With minimal logic area overhead (less than 8%), we improve the bandwidth of a 16-, a 256-, and a 1024--Floating Point Unit (FPU) baseline clusters, without Tightly Coupled Data Memory (TCDM) Burst Access, by 118%, 226%, and 77% respectively. Reaching up to 80% of the cores-memory peak bandwidth, our design demonstrates ultra-high bandwidth utilization and enables efficient performance scaling. Implemented in 12-nm FinFET technology node, compared to the serialized access baseline, our solution achieves up to 1.9x energy efficiency and 2.76x performance in real-world kernel benchmarkings.

==> source/writing_backup.tex <==
%% Abstract
% First introduce the background and problem
% As computing demands intensify, especially in data-heavy applications like machine learning, memory bandwidth has become a critical bottleneck in large-scale systems. 
% Hierarchical many-core architectures with shared L1 memory are essential for efficiently scaling these systems, providing low-latency data access while maintaining physical feasibility. 
% However, this approach, particularly in \gls{SIMD} many-core clusters, often results in hierarchical port contention during consecutive memory accesses from vector processors, leading to data serialization and performance reduction.

% Second solution and results
% We present a \gls{TCDM} burst access mechanism integrated into \gls{RVV} many-core clusters to resolve memory contention and improve bandwidth efficiency. 
% By leveraging \gls{TCDM} bursts on the request side and grouping data in a widened response channel to reduce transaction overhead, our approach mitigates port congestion without increasing the number of ports or affecting clock frequency. 
% We present \gls{TCDM} burst access, a bandwidth-optimization mechanism, with Burst Generator for sending bursts and Burst Manager to adapt burst requests for \gls{TCDM} banks.
% We add hardware parameterizeable data width on response channel to fully utilize routing resources in different design scales, futher improve performance and energy efficiency.

% Implemented in \num{12}-nm FinFET technology node, our solution achieves up to \SI{90}{\percent} energy efficiency gains and a \textbf{2.75x} performance improvement in real-world kernel benchmarking.
%%%%%%%%%%%%%%%%%%%%%%%%%%


%% Introduction
% Shared L1 \gls{TCDM} clusters with thousands of multi-precision FP units driven by small instruction-processing cores are a common architectural pattern to achieve performance and energy-efficiency~\cite{Groq} while retaining flexibility.
% A successful architectural pattern is the parallel cluster of \glspl{PE} interconnected through a low-latency, high-bandwidth, \gls{FC} crossbar to a shared memory~\cite{mempool}.
% Leveraging \gls{DMA} for data transfers becomes more prevalent in such a structure to minimize data movement overhead by avoiding the tiling of data across memory hierarchies~\cite{Kalray}.
% Moreover, employing a vectorized datapath helped to reduce instruction issues on data-parallel tasks, further enhancing \gls{FPU} utilization~\cite{spatz}.

%The Nvidia A100~\cite{nvidia_a100} and H100~\cite{nvidia_h100}, as off-the-shelf many-core designs, feature architectures where only four multi-threaded \glspl{PE} share \SI{192}{\kilo\byte} and \SI{256}{\kilo\byte} of memory per \gls{SM}, respectively.

% MemPool from the \gls{PULP} platform~\cite{mempool} extends this concept further by leveraging shared L1 memory across a 256-core cluster, and one design configuration aims to increase computing resource utilization by Vector-\gls{SIMD} support~\cite{spatz}.

%In this chapter we present the architecture of MemPool-Spatz interconnect for different core-counts. We highlight the peak memory bandwidth theoretically achievable in presence of contentions, motivating our solution.

% MemPool is an open-source, parametric, and flexible manycore architecture with a large, shared L1 \gls{SPM}~\cite{mempool}.
% The fundamental building block is the Tile, which contains multiple RV32IMA Snitch cores as basic \glspl{PE} and a subset of L1 \gls{SPM} banks.
% All Tiles in the cluster are organized into four Groups, with each Tile having four communication ports connecting to each Group.
% The TeraPool cluster~\cite{terapool} introduces a further hierarchical structure between Groups and Tiles, called SubGroup, to reduce routing complexity and improve scalability.

% In MemPool\textsubscript{N}Spatz\textsubscript{K}, the\glspl{PE} are replaced by $N$ core-complexes, each consisting of an RV32IMA Snitch and an RVV-Zve32x Spatz\textsubscript{K} vector co-processor, which includes $K$ functional units and load and store ports.
% Previous work demonstrated the high energy efficiency of the MemPool\textsubscript{64}Spatz\textsubscript{4} cluster~\cite{spatz}. However, it did not provide an in-depth performance analysis for memory-intensive workloads. 
% In this work, we further integrate Spatz into the TeraPool architecture and evaluate our designs on three configurations to cover a wide range of use cases:
% \begin{enumerate}
%     \item \textit{MinPool\textsubscript{4}Spatz\textsubscript{4}}: a \num{16}-FPU cluster, which is the smallest configuration of the MemPool cluster. It has four Spatz\textsubscript{4} separated in one Tile per Group, with a maximum \gls{VLEN} of 256 bits.
%     \item \textit{MemPool\textsubscript{64}Spatz\textsubscript{4}}: a \num{256}-FPU cluster, organized in \num{64} Tiles, with a maximum \gls{VLEN} of 256 bits.
%     \item \textit{TeraPool\textsubscript{128}Spatz\textsubscript{8}}: a \num{1024}-FPU cluster, with \num{128} Spatz\textsubscript{8} cores, with maximum \gls{VLEN} of 512 bits. \footnote{In some tables and figures, we abbreviate MinPool, MemPool as MP, TeraPool as TP, and Spatz as S for conciseness.}
% \end{enumerate}
% All configurations support \num{32}-bit floating point calculation.

%For a randomly generated vector load, the probability of targeting local or remote memory region, denoted as $p_l$ and $p_r$, depends on the total number of \glspl{PE} in the cluster:

%
% The address of a vector load can be modeled as an independent discrete random variable.
% The average memory bandwidth for a \gls{PE}, which corresponds to the expected value of this random variable, is given by:
%
% Based on the information above, we calculated the theoretical memory bandwidth for MinPool\textsubscript{4}Spatz\textsubscript{4}, MemPool\textsubscript{64}Spatz\textsubscript{4}, and TeraPool\textsubscript{128}Spatz\textsubscript{8}, summarized in the first row of Table~\ref{tab_BW_calc}.
% The results demonstrate that the vector core experiences a significant bandwidth reduction in MemPool clusters compared to its original design.
% As the cluster scales, the probability of sending a remote vector request increases, converging the average bandwidth to the $BW_r$.
% Although with the help of the new hierarchical level SubGroup in TeraPool\textsubscript{128}Spatz\textsubscript{8} cluster, the bandwidth efficiency still drops significantly to  \SI{11.75}{\percent}, severely limiting its performance on memory-intensive kernels. 
% It is important to note that these calculations are optimistic, as they do not account for inter-core conflicts and access latency.
% An urgent solution is required to mitigate this declining trend while maintaining physical feasibility in large-scale clusters.
% In most cases, vector loads follow a consecutive address pattern.
% If the number of requests can be reduced by compressing them into a narrower burst, the conflicts at the Tile-level request ports can be fully resolved without requiring additional routing resources.
% However, sending burst requests alone cannot help the narrow response channel: the data generated simultaneously would still need to be arbitrated to pass through the Tile-level hierarchical response port, suffering from the congestion again.

% An intuitive method to resolve the congestion on the response channel is to increase the communication path in the \gls{FC} interconnect between cores and \gls{TCDM} banks.
% However, this approach presents a significant challenge in physical design.
% If bandwidth is improved by a factor of $GF$, the interconnect complexity grows quadratically, by $GF^2$, due to the increased number of interconnection nodes in the \gls{FC} crossbar.

% To mitigate this, when multiple data words are destined for the same location, they can be grouped into a single transaction, reducing the routing resources required by only widening the data width. 
% Burst requests naturally align with this condition, effectively decreasing traffic and congestion in the interconnection.
% By widening the data field, this approach results in only a linear increase in routing complexity, scaling by $GF$ times instead of the quadratic growth of adding more paths.

% \subsection{Spatz \gls{VLSU}}
% A new submodule Burst Sender is added inside the \gls{VLSU} in the Spatz co-processor to send out the burst requests when detecting \textit{VLE} instructions, which are the most common in vector loading.
% Due to the L1 structure in the MemPool cluster, stride and indexed memory addresses are often scattered across \gls{TCDM} banks in different Tiles, making burst requests inefficient and challenging to implement.
% As a result, the Burst Snener submodule is configured not to send stride and indexed loads as burst requests.
% The \gls{ROB} in \gls{VLSU} on the first port is enlarged by $GF$ times to handle the increased data flow.

% The burst length is a critical parameter in burst sending.
% Unlike scalar systems, where bursts can significantly reduce the number of instructions, in a vector processor, they only reduce the number of memory transactions. 
% Additionally, long bursts occupy multiple \gls{TCDM} banks, potentially blocking requests from other cores, starving them, and negatively impacting overall performance. 
% To balance performance and \gls{QoS}, we configured the burst length to be \num{16} bytes, which fully utilizes the expanded response data channel without degrading system performance.

% The new Burst Manager block is designed and placed before the \gls{SPM} banks to adapt the \gls{TCDM} burst access:
% \begin{enumerate}
%     \item On the request channel, it takes in the burst requests, converts them into parallel \SI{32}{bit} memory requests, and forwards them to the \gls{SPM} banks.
%     An arbitrator and a small FIFO are used to hold the unadapted burst requests if multiple of them arrive simultaneously.
%     \item On the response channel, it packs the parallel response data into a packet and forwards it through the widened data field on the response channel.
% \end{enumerate}

% \subsection{Parametric response data-width}
% As the Burst Sender helps to accomplish the functionality of sending bursts, the next critical design is to increase the data
% After implementing the \gls{TCDM} burst mechanism, the primary factor limiting bandwidth is the performance of the response channel.
% An elaboration parameter, $GF$, controls the data width on the response channel to increase the design's feasibility on different cluster scales.
% In both MinPool\textsubscript{4}Spatz\textsubscript{4} and MemPool\textsubscript{64}Spatz\textsubscript{4} clusters, $GF$ is set to \num{4} to maximize the performanc, labeled as 4xRsp.
% In the TeraPool\textsubscript{128}Spatz\textsubscript{8} cluster, $GF$ is set to \num{2} to balance performance and physical design feasibility, denoted as 2xRsp.

% We evaluate the performance of \gls{TCDM} burst access implementation in our testbeds using a set of real-world kernels, chosen to cover a wide range of Arithemetric Intensity, which represents the ratio of computational operations and memory movements in bytes:
% \begin{enumerate}
%     \item \textit{\gls{DOTP}}: Scalar multiplication between two $n$-element single-precision floating-point vectors. 
%     \item \textit{\gls{FFT}}: Multi-core implementation of the Cooley-Tukey Radix-2 \gls{FFT} algorithm on $n$ complex single-precision floating-point samples.
%     An \gls{FFT} kernel is denoted as $k \times n$, where $k$ represents the number of $n$-sized \gls{FFT} kernels running in parallel.
%     \item \textit{\gls{MATMUL}}: Matrix multiplication on two $n \times n$ single-precision floating-point matrices.
% \end{enumerate}
% The evaluations are conducted through cycle-accurate \gls{RTL} simulations, with all data preloaded into the L1 memory of the testbed.

%Each Spatz\textsubscript{K} is equipped with $K$ \SI{32}{b} memory ports, matching the number of \glspl{FU}, for vector load and store operations.

% since n real-world kernels, vector stores are less frequent.
% Additionally, stores can be processed as fire-and-forget instructions, allowing \glspl{PE} to proceed with subsequent instructions immediately after issuing store requests, thus eliminating the need for acceleration.
% The solution accelerates the vector load requests only because the vector stores are less frequent in real-world kernels and can be processed as a fire-and-forgot instruction where the \glspl{PE} can continue executing the next instruction after sending out the store requests without stalls.

% Second, vector requests do not have the data information on the request channel, which prevents them from being packed into a single transfer.
% However, the parallel responses generated from a burst request must be transmitted back through the same hierarchical interconnect, becoming a new contention point.

% The second component of our proposed solution addresses the contention arising from the data produced by burst requests in the hierarchical interconnect.
%The extent of data width increase is hardware-configurable through an elaboration parameter, allowing flexibility across different cluster scales to account for the linearly increased complexity in the interconnect caused by the increased signal width.
% Because the interconnect's complexity increases linearly with the expansion of the data width, the expansion factor of the data width remains configurable to accommodate varying design scales, ensuring the optimal utilization of routing resources.
% Specifically, designs that double or quadruple the response data width are referred to as \textit{2xRsp} and \textit{4xRsp}, respectively.
% backup version without mention complexity
% By configuring the response data width to double or quadruple its size—referred to as \textit{2xRsp} and \textit{4xRsp}, respectively, this approach provides scalable solutions that efficiently adapt to various system requirements.




The results represent the average peak bandwidth of the clusters across different kernels and are plotted as dashed lines in the roofline model in Figure~\ref{fig:roofline}.
As expected, the measured bandwidth is lower than the theoretical values calculated in Table~\ref{tab_BW_calc}, but the trends remain consistent. 
The 4xRsp design restores an impressive \SI{80}{\percent} and \SI{70}{\percent} of the ideal bandwidth for MinPool\textsubscript{4}Spatz\textsubscript{4} and MemPool\textsubscript{64}Spatz\textsubscript{4}, respectively. 
TeraPool\textsubscript{128}Spatz\textsubscript{8} achieves the same bandwidth efficiency as the baseline MemPool\textsubscript{64}Spatz\textsubscript{4} with the use of 2xRsp.

The kernel results are shown in Table~\ref{tab_kernel} and marked in Figure~\ref{fig:roofline}.
In the \gls{DOTP} kernel, the burst-enabled designs exhibit a significant improvement in both utilization and performance.
The operation throughput in the MemPool\textsubscript{64}Spatz\textsubscript{4} cluster increases dramatically from \SI{61.77}{OP/cyc} to \SI{170.44}{OP/cyc}, representing an over \SI{175}{\percent} improvement. 
These gains in the \gls{DOTP} kernel align well with the roofline model, where the performance enhancement can be directly linked to the increased bandwidth efficiency in memory-bound kernels.

For the \gls{FFT} kernels, while the burst-enabled designs still exhibit significant performance improvements, these gains are limited by the frequent multi-core synchronizations inherent in the algorithm, resulting in a performance boost of over \SI{60}{\percent} for the MemPool\textsubscript{64}Spatz\textsubscript{4} cluster.

The results for the \gls{MATMUL} kernel are different due to its high arithmetic intensity, which is primarily constrained by computation rather than memory bandwidth.
However, improvements are still evident in larger clusters, where the original design suffered from poor memory bandwidth efficiency.
We observed a \SI{35}{\percent} improvement in MemPool\textsubscript{64}Spatz\textsubscript{4} and a \SI{13}{\percent} improvement in TeraPool\textsubscript{128}Spatz\textsubscript{8}, pushing the performance of compute-bound kernels in large clusters closer to their algorithmic limits.

The widened response channel leads to an increase in the logic area. 
Specifically, the logic area grows by \SI{5.5}{\percent}, \SI{7.8}{\percent}, and \SI{4.9}{\percent} in the 4xRsp MinPool\textsubscript{4}Spatz\textsubscript{4}, 4xRsp MemPool\textsubscript{64}Spatz\textsubscript{4}, and 2xRsp TeraPool\textsubscript{128}Spatz\textsubscript{8} clusters, respectively.
The physical layout of the 4xRsp design after \gls{PNR} is shown in Figure~\ref{fig:layout}.

The left part of Figure~\ref{fig:power-area} shows the logic area breakdown for the original and 4xRsp configurations of the MemPool\textsubscript{64}Spatz\textsubscript{4} cluster.
The widened data field results in a total area increase of \SI{7.76}{\percent}, primarily due to the interconnection, \gls{VLSU}, and the newly introduced Burst Manager blocks.
While an increase in this area adds complexity, it directly contributes to the improved bandwidth and performance seen in the burst-enabled designs.
The trade-off between area and performance becomes evident in memory-bound kernels, where the additional hardware significantly boosts throughput and efficiency, as demonstrated in the \gls{DOTP} kernel.

A detailed power breakdown for the \gls{MATMUL} kernel was extracted to analyze the additional power consumption, as shown in the right part of Figure~\ref{fig:power-area}.
The increased power usage is concentrated in the \gls{VLSU}, interconnection, \gls{TCDM} banks, and the Burst Manager block, confirming that faster data transfers are the primary cause of the additional power draw.
While the power consumption increases, this is expected due to the enhanced core utilization enabled by the 4xRsp and 2xRsp designs.




Although the burst-enabled configurations demonstrate higher power usage, they achieve significant energy efficiency gains, particularly in memory-bound kernels.
For instance, the \gls{DOTP} kernel sees a \SI{90}{\percent} improvement in energy efficiency due to the shorter execution time, which compensates for the additional power used.
However, kernels such as \gls{FFT}, constrained by synchronization overhead, show only marginal energy efficiency gains despite the increased bandwidth.
The \gls{MATMUL} kernel, being compute-bound, sees minimal benefit from faster memory transfers, leading to a slight drop in energy efficiency for larger data sizes.

From a physical design perspective, the area and power increases remain within acceptable limits, allowing the system to maintain high performance without exceeding thermal or power budget constraints. 
The careful balance between area growth and bandwidth recovery ensures that the clusters maintain scalability even with the additional hardware, especially in larger designs like TeraPool\textsubscript{128}Spatz\textsubscript{8}.



% As the cluster scales up, the probability that requests target addresses in remote hierarchies increases, resulting in more requests requiring arbitration at hierarchical interconnection ports and consequently decreasing bandwidth utilization.
% Only \SI{11.75}{\percent} of the peak \glspl{VLSU} bandwidth is achieved in the \num{1024}-FPU vector cluster.

% When detecting a consecutive vector request pattern, it issues a burst request with a burst length of $K$ words.
% It halts the ongoing request process and issues a burst request with a burst length of $K$ words when detecting a consecutive vector request pattern, aligning with the theoretical \gls{VLSU} peak bandwidth.
% The \gls{NUMA} architecture in large clusters cannot guarantee the ordering between memory requests and responses.
% Therefore, a \gls{ROB} is implemented at each memory interface in our testbed clusters to ensure proper reordering.
% Since the \gls{NUMA} L1 architecture in the MemPool-Spatz clusters does not guarantee the ordering between memory requests and responses, a \gls{ROB} is implemented at each memory interface.
% To accommodate for the higher transfer frequency from burst requests, the depth of \gls{ROB} needs to be increased.

% As a result, lower bandwidth utilization is observed in the MP\textsubscript{128}Spatz\textsubscript{8} cluster.
% On larger cluster scales, interconnection complexity is constrained by physical design feasibility, and bandwidth is limited due to increased arbitration among more cores at shared ports~\cite{terapool}.
% The \gls{SIMD} memory accessing pattern discussed earlier in~\cref{sec:introduction} hides this reduction: all requests are serialized through the same hierarchical port due to contention, presenting the same \textit{remote-Hierarchy} bandwidth of \SI{4}{Bytes/cyc} in the testbed clusters.
% % making no differences in \textit{remote-Hierarchy} visits in different design scales.
% The higher \textit{local-Tile} bandwidth in our MP\textsubscript{128}Spatz\textsubscript{8} testbed leads to a slightly higher hierarchical average bandwidth, compared to a smaller MP\textsubscript{64}Spatz\textsubscript{4} testbed cluster.
% However, the bandwidth utilization still decreases because of the more \gls{VLSU} ports in the Spatz\textsubscript{8} processor.

% Implementing the \gls{TCDM} burst access results in an increase in the logic area within the testbed clusters.
% A logic area growth of \SI{5.5}{\percent}, \SI{7.8}{\percent}, and \SI{4.9}{\percent} is observed in MP\textsubscript{16}Spatz\textsubscript{4}, MP\textsubscript{64}Spatz\textsubscript{4} and MP\textsubscript{128}Spatz\textsubscript{8}, respectively.


% As a result, the $128\times128\times128$ \gls{MATMUL} kernel's performance is limited by the memory bandwidth. showing a \SI{62}{\percent} improvement with \textit{GF2} design 
% In the \gls{MATMUL} kernel, constrained by memory bandwidth, the \num{128}-sized kernel shows a \SI{62}{\percent} improvement with \textit{GF2} implemented, while 


% Adopting the \gls{TCDM} burst access mechanism increases the power consumption in general, primarily due to the higher \gls{FPU} utilization.
% With the performance improvements of \SI{176}{\percent}, energy efficiency increases by up to \SI{90}{\percent} in all memory-bound kernels compared to the baseline testbed clusters.
% However, a slight reduction of \SI{10}{\percent} in energy efficiency is observed in $256\times 256\times 256$ \gls{MATMUL} kernel on the MP\textsubscript{64}Spatz\textsubscript{4} testbed with \textit{GF4} design.
% A power breakdown is shown in the right part of~\cref{fig:power-area} to analyze the causes of this reduction.
% The increased power consumption in the \gls{VLSU}, \gls{SPM} banks and interconnection logic indicates a higher data transfer rate due to the increased hierarchical average bandwidth.
% However, the compute-bound kernel does not benefit from the faster data loading in terms of performance, which leads to a drop in energy efficiency.

% In our analysis, the roofline model serves as a framework to evaluate the effectiveness of \gls{TCDM} burst access mechanism in improving bandwidth utilization and performance across different real-world kernels, each exhibiting different arithmetic intensities:


The performance and energy efficiency improve by up to \SI{106}{\percent} and  \SI{45}{\percent} in MP\textsubscript{4}Spatz\textsubscript{4} respectively compared against the original cluster.
In a larger MP\textsubscript{64}Spatz\textsubscript{4} cluster, it boosts the performance and energy efficiency up to \SI{176}{\percent} and \SI{90}{\percent}, with less than \SI{8}{\percent} area overhead and no impact on the operating frequency.
Additionally, it scales well on MP\textsubscript{128}Spatz\textsubscript{8} cluster, achieving up to \SI{80}{\percent} performance improvement and \SI{40}{\percent} energy efficiency gain by doubling the response data width.

Our design suggests a viable solution for addressing memory bandwidth bottleneck in large-scale many core vector clusters, offering substantial performance and energy efficiency improvements while maintaining physical feasibility.


==> tab/meas_bw.tex <==
\begin{table}[]
\centering
\caption{Memory Bandwidth: Bandwidth Test and Comparison.}
\label{tab_BW_meas}
\begin{tabular}{llrrr}
\hline
                                  &                & \multicolumn{1}{l}{\textbf{MP\textsubscript{4}Spatz\textsubscript{4}}} & \multicolumn{1}{l}{\textbf{MP\textsubscript{64}Spazt\textsubscript{4}}} & \multicolumn{1}{l}{\textbf{TP\textsubscript{128}Spatz\textsubscript{8}}} \\
\textbf{Ideal}                    &                & 16.00                                  & 16.00                                   & 32.00                                    \\ \hline
\multirow{2}{*}{\textbf{Baseline}} & BW {[}B/cyc{]} & 6.00                                   & 3.42                                    & 3.76                                     \\
                                  & Efficiency     & 37.50\%                                & 21.38\%                                 & 11.75\%                                  \\ \hline
\multirow{3}{*}{\textbf{2xRsp}}   & BW {[}B/cyc{]} & 7.34                                   & 6.42                                    & 6.64                                     \\
                                  & Efficiency     & 45.88\%                                & 40.13\%                                 & 20.75\%                                  \\
                                  & Improvement    & +22.33\%                                & +87.72\%                                 & +76.60\%                                  \\ \hline
\multirow{3}{*}{\textbf{4xRsp}}   & BW {[}B/cyc{]} & 13.11                                  & 11.15                                   & 11.24                                    \\
                                  & Efficiency     & 81.94\%                                & 69.69\%                                 & 35.13\%                                  \\
                                  & Improvement    & +118.50\%                               & +226.02\%                                & +198.94\%                                 \\ \hline
\end{tabular}
\end{table}
